Collaborative Split Federated Learning with Parallel Training and Aggregation

Federated learning (FL) operates based on model exchanges between the server and the clients, and it suffers from significant client-side computation and communication burden. Split federated learning (SFL) arises a promising solution by splitting the model into two parts, that are trained sequentially: the clients train the first part of the model (client-side model) and transmit it to the server that trains the second (server-side model). Existing SFL schemes though still exhibit long training delays and significant communication overhead, especially when clients of different computing capability participate. Thus, we propose Collaborative-Split Federated Learning~(C-SFL), a novel scheme that splits the model into three parts, namely the model parts trained at the computationally weak clients, the ones trained at the computationally strong clients, and the ones at the server. Unlike existing works, C-SFL enables parallel training and aggregation of model's parts at the clients and at the server, resulting in reduced training delays and commmunication overhead while improving the model's accuracy. Experiments verify the multiple gains of C-SFL against the existing schemes.

==> scheme.tex <==
\section{Pa- SFL scheme design - Do not read}\label{sec:design}
We present the phases of the Pa-SFL scheme, a synchronous split-federated learning scheme, which aims to reduce the training time of a global DNN model.
The \textit{core idea} of Pa-SFL is to train in parallel both the global device-side and server-side models. The device-side model's training is accelerated by enabling \textit{weak} devices to offload layers to \textit{strong} devices. The strong devices, namely local-aggregators, compute a partial-loss by utilizing the already offloaded layers by their assigned weak devices. Concurrently, the server-side model's training is also accelerated by distributing computation load to strong devices (local-aggregators), rather than transferring it to the server.
%Then follows the aggregation of these local models (update of device-side model) and the update of the server-side model repeatedly until the global DNN model is accurate enough.

\subsection{Initialization}
The AP collects the network statistics and determines the cut layer $v$ in order to partition the global DNN model $W$ into two parts: the device-side and the server-side models, which remain unchanged throughout the entire training process. 
Both of them are initialized with random weights.
In case $v=V$, then \mbox{Pa-SFL} degrades to the typical federated learning scheme.
Also, the AP determines the placement of the local-aggregators and the offloaded layers per device for the first training round.
Finally, AP broadcasts $W^d$ to all participating devices. (\ref{eq:dmodeldistribution}) to initiate the training process.

Let $W^d(t,\pi)$ ($W^s(t,\pi)$) denote the device-side (server-side) model at round $t$ and epoch $\pi$.
Let also $w^d_{n}(t , \pi=1)$ denote the local model of device $n$ at local epoch $\pi$ and round $t$.
\begin{equation}\label{eq:dmodeldistribution}
    w^d_{1, n}(t=1, \pi=1) \leftarrow W^d(t=1, \pi=1) , \forall n \in N
\end{equation}
\subsection{Batch training}
For each batch $b_n \in B$:

\subsubsection{Local models's forward propagation}
Each device $n$ draws a \textit{mini-batch} $b_n \subseteq D_n$ from its own dataset.
It then executes FP on its respective local model $w^d_n$ for its assigned layers ($x_{i,j,n}, \forall i, ~i==n$) and obtains smashed data. %$S^{x_{n,j,n}}_{\pi n}(t)$.
Afterwards, it transmits the computed smashed data and corresponding labels to its assigned local aggregator $k(n)$ to continue the FP process up to the cut layer $v$ and receive the resulting smashed data:
\begin{equation}\label{eq:smashdata}
    S^{v}_{n}(t,\pi) \leftarrow \sum_{b_n}^{D_n} f(b_n, w^d_{n}(t,\pi)), ~~ \forall n \in N
\end{equation}
where $f(b_n, w^d_n)$ represents the mapping function between input dataset and output given local model weights $w^d_n$. These smashed datas $S^{v}_{n}(t,\pi)$ are sent to the AP by the local-aggregators for the server-side model's update.
%In case a device $n$ is assigned an individual cut layer smaller than the global cut layer, transmits the smashed data $S^{V_cn}_{cn}{\pi n}(t)$ to its computation server $S_n$.
%Then $S_n$ continues the FP from $V_{cn}$ until $V_c$ and computes the $S^{V_c}_{\pi n}(t)$, which is then transmitted to the AP.

\subsubsection{Partial loss computation}
Each local-aggregator $k$ computes the local-loss for each assigned device $n$ (where $k(n)=k$) up to layer $v$, denoted by $L_n^v (w^d_n)$. 
It then averages these local-losses to compute the partial-loss.
This partial-loss is used to initiate the BP process for each offloaded layer to the local-aggregator ($x_{i,j,k}==1$).

\subsubsection{Local models's backward propagation}


\subsubsection{Global server-side model's update}
The AP receives and aggregates the smashed data of the participating devices by the local-aggregators:
\begin{equation}\label{eq:smashdataaggr}
S^v_{}(t,\pi)= [S^v_{\1}(t, \pi); S^v_{\2}(t, \pi);..S^v_{N}(t, \pi)] 
\end{equation}
Then feeds the aggregated smashed data into the server-side model $W^s(t)$.
As a result, the predicted result ($y^p$) from the server-side model:

\begin{equation}\label{eq:predictedres}
y^p_\pi(t)= f(S^v_{\pi}(t); W^d(t) + W^s(t)), \forall \pi \in \Pi
\end{equation}

After (\ref{eq:smashdata})(\ref{eq:predictedres}) the one epoch FP process of the global model $W$ is completed.
Subsequently, the global loss $L(W)$ and the averaged gradients of the loss $(\nabla L(W) )$ are computed since both the ground truth labels and the predicted results (\ref{eq:predictedres}) are available to the AP.

\subsubsection{Server-side model's back propagation}
Following, the AP performs BP on the server-side model using the SGD algorithm\textbf{CITE} starting from the last layer until the global cut layer inline with the chain rule for gradient calculation:

\begin{equation}\label{eq:bpserver}
    W^s_{\pi+1}(t) = W^s_{\pi}(t) - \eta_s \nabla L(W^s_{\pi}(t))
\end{equation}
where $\eta_s$ denotes the learning rate of the server-side model updates.
When the BP process proceeds to the cut layer, the gradients of each smashed data received is calculated and sent back to the originator device.
\subsubsection{Local models's back propagation}
Finally, each device receives the gradients of the smashed data it sent and updates the respective weights of its local model using the SGD algorithm:

\begin{equation}\label{eq:bplocal}
    w^d_{\pi+1 n}(t) =  w^d_{\pi n}(t) - \eta_d \nabla L(w^d_{\pi n}(t))
\end{equation}

where $\eta_d$ denotes the learning rate of device-side model.

In case, a device $n$ is assigned an individual cut layer smaller than the global cut layer, the respective computation server $S_n$ is responsible to perform the BP process until $V_{cn}$.
When the computation server obtains the gradients of the smashed data until layer $V_{cn}$, transmits them to the corresponding device $n$ in order to continue the BP process for the remaining layers.
With (\ref{eq:bpserver})(\ref{eq:bplocal}) the one epoch BP process of each local model is completed.

\subsubsection{Global device-side model's update}
To conclude the current round, after $\Pi$ local epochs are completed, all participating devices upload their respective local model weights ($w^d_n$) to the AP.
Then the AP is responsible to update the device-side model using all local models via the well known FedAVG algorithm~\textbf{CITE} based on the amount of data each device possesses (\ref{eq:fedavg}).
\begin{equation}\label{eq:fedavg}
    W^d(t+1)= \frac{\sum_{n=1}^{N}  |D_n| w^d_{\Pi n}(t)}{\sum_{n=1}^{N}  |D_n|}
\end{equation}

With (\ref{eq:bpserver})(\ref{eq:fedavg}) the global model $W$ is updated during the round $t$. The AP is responsible to terminate the training process, when the global model converges.
%\subsection{Device limitations}
\subsection{Training latency}
The total training latency of Pa-SFL equals with the.
We aim to analyze the latency per stage during each epoch as described in sec.\ref{sec:design}.B. 
For notation simplicity, we omit $t$ and $\pi$ in this subsection.

\subsubsection{Local models's forward propagation}
In the Pa-SFL scheme, the AP waits for the smashed data of each participating device.
The latency incurred in current step results from the slowest forward propagation over all local models until the global cut layer $V_c$.
We take into account that a device $n$ may require assistance from another device $S_n$, yet we assume that the transmission latency of smashed data between devices is negligible and is not considered in current analysis(\ref{eq:fpdelay}). We denote $K(S^v)$ as the computation workload (in FLOPS) required to compute the smashed data until cut layer $V_c$.

\begin{equation}\label{eq:fpdelay}
    D^{fp}_d = \max\limits_{n \in N} (\frac{K(S_n^{1 - V_{cn}})}{P_n} + \frac{K(S^{V_{cn} - V_c}_n)}{P_{S_n}})
\end{equation}

\subsubsection{Server side model's update}
The server-side model's update latency consists of three parts: (a) the aggregation of smashed datas received (b) server-side model's forward propagation until last layer and loss computation (c) server-side model's backward propagation until the global cut layer.
The delay of devices's smashed datas aggregation at the AP is negligible(a), since it involves simple concatenation.
The second part includes the time required to perform FP on the server-side model, where the total workload of comprises the aggregated smashed data of each participating device

\begin{equation}\label{eq:serverfpdelay}
     D^{fp}_s = \frac{N' *K(S^{V-V_c})}{P_s}
\end{equation}
Similarly, the third part involves the time required to perform BP until the global cut layer and to compute the respective gradients(\ref{eq:serverbpdelay}).
\begin{equation}\label{eq:serverbpdelay}
     D^{bp}_s = \frac{K(\nabla S^{V_c-V})}{P_s}
\end{equation}
Also, we assume that the smashed data gradients are broadcasted to the devices simultaneously or with negligible time difference.
\subsubsection{Local models's backward propagation}
After the devices receive the gradients of the smashed datas, continue the BP from their individual cut layer until the first layer to update the respective local model's weights.
\begin{equation}\label{eq:bpdelay}
    D^{bp}_d = \max\limits_{n \in N} (\frac{K(\nabla S^{V_c- Vcn}_n)}{P_{S_n}} + \frac{K(\nabla S^{Vcn-1}_n)}{P_n})
\end{equation}

After $\Pi$ epochs, the devices upload their local models to the AP.
Also, the aggregation of the local models using the FedAVG algorithm requires minimal computation time\textbf{CITE}.
Besides that, it is independent to the cut layers selections.
Hence, the overall latency in one round $t$ equals with:
\begin{equation}\label{eq:bpdelay}
    D(t) =  \sum_{\pi=1}^{\Pi}D^{fp}_d(\pi) + D^{fp}_s(\pi) + D^{bp}_s(\pi) + D^{bp}_d(\pi)
\end{equation}
The global cut layer affects the computation workload distribution between the devices and the AP.
A deep global cut layer means light computation workload for the edge server and heavy for the devices, while a shallow ones the opposite.


==> workflow.tex <==
\section{Training workflow in C-SFL}
The training workflow in C-SFL is orchestrated by the server, usually an edge-server that is connected with the clients via wireless links.
The server collects the clients's statistics (computing capability, available memory, wireless connectivity) and makes the orchestration decisions in a centralized fashion.
Specifically, the server decides and informs the clients for the: the selected cut $v$ and collaborative $h$ layers.

The network bootstraps by initializing the client-side ($W^d$) and the server-side ($W^s$) models randomly.
Then, each client downloads the $W^d$, which is split into the weak-side $W^w$ and the aggregator-side $W^a$ models at the collaborative layer $h$, from the server to initiate the training process.
Every client $n$ performs FP on its $w^w_n$ and then transmits the collaborative layer's $h$ activations and input labels to its assigned local-aggregator.
Each local-aggregator $k$ performs FP both on its own $w^w_k$ and $w^a_k$ and computes the local-loss $ll_k(w^a_k)$ along with the respective gradients $\nabla ll_k(w^a_k)$.
Also, transmits to the server the cut layer's activations.
Then, completes the BP process on both the $w^a_k$ and $w^w_k$.
Concurrently, the local-aggregators perform the same processes for their assigned clients' $i \in S_k$ aggregator-side models (see Fig.\ref{fig:workflow}).
They, also transmit the collaborative layer's $h$ gradients back to the corresponding client(s) to complete the BP process and update the respective weak-side model(s).

In parallel, upon receiving the cut layer's activations, the server then updates the server-side models $W^s_n \forall n \in N$ (FP and BP) and computes the accuracy (or loss) $gl(W^s_n)$ using the global-loss function at the output layer.
This workflow is repeated for all $B$ batches of data (1 epoch).
To conclude the current epoch, the server aggregates the server-side models to compute the global server-side model for the next epoch. 
Similarly, the local-aggregator aggregates the aggregator-side models of its own assigned clients (see Algorithm \ref{alg:CSFLepoch}).
\begin{algorithm}[tbp]
\caption{Collaborative Split Federated Learning}
\label{alg:CSFL}
\begin{algorithmic}[1]
\State Initialize \( W^S_t \) (global server-side model)
\State Initialize \( W^D_t \) (global client-side model)
\While{round $t \neq T$}
    \State $L(W) \leftarrow L(W^D_t;W^S_t)$
    \If{$L(W) \leq L_{thr}$}
    \State Collect client's $n$ statistics, $\forall  n \in N$
    \State Decide $Local-aggregator(n),\forall  n \in N$ \State Decide cut layer $v$, collaborative layer $h$
    \State $W^S_{t}, W^D_t \leftarrow$\text{C-SFL-Round ($W^S_{t},W^D_t $,$K$,$v$,$h$)}
    \State $t \leftarrow t+1$
    \State Send ($n$,$W^D_{t}$), $\forall  n \in N$
    \Else
    \State $t \leftarrow T$
    \EndIf
    %\State \textbf{end if}
\EndWhile
\State \textbf{end while}
\end{algorithmic}
\end{algorithm}
\setcounter{ALG@line}{0} % Reset line numbering
\begin{algorithm}[!tbp]
\caption{C-SFL-Round}\label{alg:CSFLepoch}
\textbf{Input:} server-side model $W^S_t$, client-side model $W^D_t$, local-aggregator $S$ ,cut layer $v$, collaborative layer $h$, learning rate $\eta$ \\
\textbf{Output:} server-side model $W^S_{t+1}$, client-side model $W^D_{t+1}$
\begin{algorithmic}[1]
%\textbf{Input:} server-side model,
\State Initialize \( W^S_t \) (global server-side model)
\State Initialize \( W^w_t \) (global weak-side model)
\State Initialize \( W^w_t \) (global aggregator-side model)
\While{epoch \( \pi \neq \Pi \)}
    \For{each client \( n \) in parallel}
        \If{$local-aggregator(n) \neq n$}
            \State \( (Ah_{n,t}) \leftarrow \text{FP}(w^w_{n,t}, b_n) \)
            \State Send($local-aggregator(n)$, $(Ah_{n,t})$)
            \State Wait($local-aggregator(n)$, $\nabla (Ah_{n,t})$)
            \State BP($w^w_{n,t}$, $\nabla (A_{n,t})$)
        \Else
            \For{each local-aggregator \( k \in K \) in parallel}
                \State \( (Ah_{k,t}) \leftarrow \text{FP}(w^w_{k,t}, b_k) \)
                \State \( (Av_{n,t}) \leftarrow \text{FP}(w^a_{n,t}, Av_{n,t}) \), \forall \( n \in S_k \)
                \State Send(server, $Av_{n,t}$), \forall \( n \in S_k \)
                \State Compute $\hat{Y}_n$ with $a_n$, \forall \( n \in S_k \)
                \State Local-Loss (\( Y_n \), \( \hat{Y}_n \)) \& $\nabla ll_n(w^a_n)$, \forall \( n \in S_k \)
                \State BP($w^a_{n,t}$, $\nabla ll_n(w^a_n)$)
                \State Send($n$, $\nabla ll_n(w^a_n)$)
                \State Wait($local-aggregator(n)$, $\nabla (Ah_{n,t})$)
                \State BP($w^w_{n,t}$, $\nabla (A_{n,t})$)
            \EndFor
        \EndIf
    \EndFor
    \State Concurrently, the server:
    \State Wait($Av_{n,t}$), \forall \( n \in N \)
    \State $\hat{Y}_n$ \leftarrow FP($W^s_{n,t}$,$Av_{n,t}$), \forall \( n \in N \)
    \State Global-Loss (\( Y_n \), \( \hat{Y}_n \)) \& $\nabla gl_n(w^s_{n,t})$, \forall \( n \in N \)
    \State BP($w^s_{n,t}$, $\nabla ll_n(w^s_{n,t})$)
    \State \( W^S_{\pi+1} \leftarrow W^S_\pi - \eta \frac{n_k}{n} \sum_{i=1}^K \nabla \ell_i(W^S_t; A^S_t) \)
\EndWhile
\State \textbf{end while}
\State \( W^S_{t+1} \leftarrow W^S_t - \eta  \sum_{n=1}^N \nabla \ell_n(W^S_t; A^S_t) \) 
\State \( W^D_{t+1} \leftarrow W^D_t - \eta \sum_{n=1}^N \nabla \ell_n(W^D_t; A^S_t) \) 
\end{algorithmic}
\end{algorithm}
\begin{comment}
\begin{algorithm}\label{alg:Algorithm_Pa-SFL}
\caption{Collaborative Split Federated Learning}
\begin{algorithmic}[1]
    \State Every client $n$ performs FP for its assigned layers and offloads the remaining layers (until the cut layer $v$), along with the corresponding activations and input labels to its assigned local-aggregator.
    \State The local-aggregators continue the FP process for the received layers for each assigned client. 
    Then, initiate the BP process using Stochastic Gradient Descent (SGD) for the offloaded layers and transmit the corresponding gradients to the assigned clients.
    \State Concurrently with step 2, the local-aggregators transmit the  the cut layer's activations to the edge-server.
    \State The edge-server concatenates the activations received from the local-aggregators and inputs it into $W^s$ for FP. Subsequently, $W^s$ is updated and the averaged gradients of the loss function $\nabla L(W)$ are computed. The AP performs BP from layer $V$ to $v$ on $W^s$ using SGD.
    \State Concurrently with step 4, each client $n$ continues the BP process until the first layer.
\end{algorithmic}
\end{algorithm}
\end{comment}
%When $B$ Batches are processed the local-aggregator aggregates the already offloaded layers from its assigned clients to a partial-client-side-model as shown in Figure \ref{fig:workflow}.

After $\Pi$ local epochs, the $K$ local-aggregators transmit to their assigned clients $i \in S_k, ~\forall k \in K$ their aggregator-side model.
Then, each client $n$ concatenates both its own weak-side $w^w_n$ and the received aggregator-side $w^a_k$ model to compute their client-side model ($w^d_n \rightarrow w^w_n+w^a_k$), and transmit it to the server.
The server updates the global client-side model via the FedAvg algorithm and transmits it back to the clients for the next training round.
The number of batches $B$ per epoch depends on the client's datasets size, while $\Pi$ is the same for each training round $t$.
The aforementioned procedure is repeated for a number of training rounds, until the global model converges (reaches target loss), as depicted in Algorithm \ref{alg:CSFL}.

Moreover, there is an inherent coupling between the FP and the BP process.
Specifically, when a client $n$ is assigned to a local aggregator $k$, both the FP and the BP process take place into the same aggregator.
Thus, the local-aggregator should allocate memory for both the smashed data of each layer received, that is required during the FP process and similar amount of memory for the gradients during the BP process.
We denote $f_j$ (in Mbytes) the amount of memory needed for the layer $j$.
Practically the amount of memory needed per layer $j$ differs but we make this assumption for simplicity.
\begin{figure}
\hspace{-0.40cm}\includegraphics[angle=270,trim={4cm 0cm 3cm 10cm},clip,scale=0.46]{figures/workflow.eps}
\caption{The workflow for the processing of B batches (one epoch).
  After B batches the local-aggregator updates (FP and BP) the aggregator-side model while the server updates the server-side model in parallel.}
\label{fig:workflow}
\end{figure}
\begin{comment}
\subsection{Message and computation overhead}
Each client $n$ may send its statistics to other client $n'$, concerning its computation capacity/availability. The Statistics Messages are denoted by $SM_{n,n'}$ and require specific amount of rate (in bps).
Statistics messages operate as a heartbeat mechanism to ensure the liveliness of the link.
Also, each client $n$ may accommodate additional computation overhead, other than its own local model. Specifically, one or more clients $n'$ may need assistance to compute their own local model from client $n$ and send the forward propagation gradients until the cut layer computed.
The Computation Messages are denoted by $CM_{n, n'}$ and also require specific amount of rate, which traditionally is bigger than the statistics messages.
We also define $CM'_{n, n'}$ as the Computation Messages, that include the back propagation gradients from last until the cut layer, computed from $n'$ and sent to $n$.

Lastly, we define Parameter Messages $PM_{n, n'}$ sent from $n$ to $ps$, which include the updated local model weights of $w_n$.
Also, $PM'{ps, n}$ represent the aggregated weights sent from parameter server to the client $n$.
\end{comment}
%\begin{comment}
\begin{table}
\caption{Notation Table}
\begin{tabularx}{\textwidth}{{}{}}
\toprule
  $a_j$ & Number of parameters of layer $j$ (in bits) \\
  $B$ & Number of batches \\
  $D(\cdot)$ & Training latency function\\
  %$D_n$ & Dataset of client $n$ \\
  $f_j$ & Computation workload of layer $j$ (in MFLOPS)\\
  $h$ & Collaborative layer\\
  $K$ & Set of aggregators \\
  $N$ & Set of clients \\
  $g_j$ & Gradients of layer $j$ (in bits)\\
  %$L(W)$ & Average loss of model $W$\\
  %$L_{thr}$ & Loss threshold\\
  %$k_n$ & Local-aggregator's placement at client $n$\\
  %$m_n$ & Available memory of client $n$\\
  %$m_s$ & Available memory of edge server\\
  $p_n$ & Computing capability of client $n$ (in MFLOPS)\\
  $p_i$ & Computing capability of aggregator $i$ (in MFLOPS)\\
  $p_s$ & Computing capability of edge server(in MFLOPS)\\
  $r_{i,j}$ & Bandwidth of link between clients $i$ and $j$ (in bits/sec)\\
  %$T$ & Number of training rounds
  $v$ & Cut layer \\
  %$w_n(t)$ & Local model of client $n$ at training round $t$\\
  %$W^d(t)$ & Global client-side model at training round $t$\\
  %$W^s(t)$ & Global Server-side model at training round $t$\\
  %$W(t)$ & Global model at training round $t$\\
  $x_{i,n}$ & Assignment of client $i$ to aggregator $n$ \\
  $\sum x_{i,n}$ & number of clients assigned to aggregator $n$ \\
  %$\Pi$ & Number of local epochs
\bottomrule
\end{tabularx}
\end{table}
%\end{comment}
